Scalable Hash-Based Estimation of Divergence Measures

We propose a scalable divergence estimation method based on hashing. Consider two continuous random variables $X$ and $Y$ whose densities have bounded support. We consider a particular locality sensitive random hashing, and consider the ratio of samples in each hash bin having non-zero numbers of Y samples. We prove that the weighted average of these ratios over all of the hash bins converges to f-divergences between the two samples sets. We show that the proposed estimator is optimal in terms of both MSE rate and computational complexity. We derive the MSE rates for two families of smooth functions; the H\"{o}lder smoothness class and differentiable functions. In particular, it is proved that if the density functions have bounded derivatives up to the order $d/2$, where $d$ is the dimension of samples, the optimal parametric MSE rate of $O(1/N)$ can be achieved. The computational complexity is shown to be $O(N)$, which is optimal. To the best of our knowledge, this is the first empirical divergence estimator that has optimal computational complexity and achieves the optimal parametric MSE estimation rate.

==> known_support.tex <==
\section{\color{red} Known Support (To be updated)}

For simplicity assume that the density support is $[0,1]^d$, but we later discuss that all the results hold true for any bounded density support. Let $l$ be a positive integer. We divide each axis to $l$ parts. $L:=l^d$ is the total number of partitions, and   Let $Q_i, 0\leq i \leq L$ be the set of points from $Z$ in partition $i$. 
Also define $N_i$ and $M_i$ as the number of points of the sets $X$ and $Y$ among $Q_i$, respectively. Moreover, we represent the support of partition $i$ by $B_i$. Then an estimator for R\'{e}nyi divergence is

\begin{equation}\label{est_Renyi_def0}
\widetilde{D}_{\alpha}(X,Y):=\frac{1}{(\alpha-1)}\log \of[\frac{\eta^{\alpha}}{M}\sum_{\substack{i\leq L \\ M_i>0}}\left(\frac{N_i}{M_i+1}\right)^\alpha M_i],
\end{equation}
where $\eta:=M/N$. 
